Counterfactual Data Augmentation improves Factuality of Abstractive Summarization

Abstractive summarization systems based on pretrained language models often generate coherent but factually inconsistent sentences. In this paper, we present a counterfactual data augmentation approach where we augment data with perturbed summaries that increase the training data diversity. Specifically, we present three augmentation approaches based on replacing (i) entities from other and the same category and (ii) nouns with their corresponding WordNet hypernyms. We show that augmenting the training data with our approach improves the factual correctness of summaries without significantly affecting the ROUGE score. We show that in two commonly used summarization datasets (CNN/Dailymail and XSum), we improve the factual correctness by about 2.5 points on average

==> exp_figure/cnndm.tex <==
training_eval_cnn_dailymail


train
Wall time,Step,Value


training_eval_cnn_dailymail_categorical
Wall time,Step,Value

train (1)
Wall time,Step,Value


==> exp_figure/xsum.tex <==
training_eval_xsum
Wall time,Step,Value

train
Wall time,Step,Value


training_eval_xsum_wn_tagged
Wall time,Step,Value

train (1)
Wall time,Step,Value

